Demystifying AI Platform Design for Distributed Inference of Next-Generation LLM models

Large language models (LLMs) have shown remarkable performance across a wide range of applications, often outperforming human experts. However, deploying these gigantic models efficiently for diverse inference use cases requires carefully designed hardware platforms with ample computing, memory, and network resources. With constant innovation in LLM serving optimizations and model architecture evolving at breakneck speed, the hardware requirements to meet Service Level Objectives (SLOs) remain an open research question. To answer the question, we present an analytical tool, GenZ, to efficiently navigate the relationship between diverse LLM model architectures(Dense, GQA, MoE, Mamba), LLM serving optimizations(Chunking, Speculative decoding, quanitization), and AI platform design parameters. Our tool estimates LLM inference performance metrics for the given scenario. We have validated against real hardware platforms running various different LLM models, achieving a max geomean error of 5.82.We use GenZ to identify compute, memory capacity, memory bandwidth, network latency, and network bandwidth requirements across diverse LLM inference use cases. We also study diverse architectural choices in use today (inspired by LLM serving platforms from several vendors) to help inform computer architects designing next-generation AI hardware accelerators and platforms. The trends and insights derived from GenZ can guide AI engineers deploying LLMs as well as computer architects designing next-generation hardware accelerators and platforms. Ultimately, this work sheds light on the platform design considerations for unlocking the full potential of large language models across a spectrum of applications. The source code is available at https://github.com/abhibambhaniya/GenZ-LLM-Analyzer . Users can also be tried it on at https://genz-llm-analyzer.streamlit.app/ without any setup on your web browser.

==> Figures/Tex/ICN_BW_scaling.tex <==
\begin{figure}[h!]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=25em]{Figures/Sources/nvlink_BW_scaling_prefill.pdf}
        % \vspace{-2em}
        \text{(a) Prefill \checkbox}
        \label{fig:nvlink_BW_scaling_prefill}
    \end{subfigure}
    
    % \vspace{1em} % Adjust the vertical spacing as needed
    
    \begin{subfigure}
        \centering
        \includegraphics[width=25em]{Figures/Sources/nvlink_BW_scaling_decode.pdf}
        % \vspace{-2em}
        \text{(b) Decode \xbox}
        \label{fig:nvlink_BW_scaling_decode}
    \end{subfigure}
    
    \vspace{-0.5em} % Adjust the vertical spacing as needed

    \caption{Scaling interconnect network BW for platform running code-generation use case. GPT3 and GPT4 uses 24(TP:12+PP:2) and 84(TP:21+PP:4) NPUs respectively.}
    \vspace{-1em}
    \label{fig:icn_bw_scaling}
\end{figure}

==> Figures/Tex/ICN_LL_scaling.tex <==
\begin{figure}[!h]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=25em]{Figures/Sources/nvlink_latency_scaling_prefill.pdf}
        % \vspace{-0.5em}
        \text{(a) Prefill \xbox}
        \label{fig:nvlink_latency_scaling_prefill}
    \end{subfigure}
    
    % \vspace{1em} % Adjust the vertical spacing as needed
    
    \begin{subfigure}
        \centering
        \includegraphics[width=25em]{Figures/Sources/nvlink_latency_scaling_decode.pdf}
       % \vspace{-2em}
        \text{(b) Decode \checkbox}
        \label{fig:nvlink_latency_scaling_decode}
    \end{subfigure}
    
    % \vspace{1em} % Adjust the vertical spacing as needed
    \vspace{-0.5em} % Adjust the vertical spacing as needed

    \caption{Scaling Interconnect network link latency for a model with code-generation use case. GPT3 uses 24 accelerators with TP:12+PP:2, and GPT4 uses 84 accelerators with TP:21+PP:4. }
    \vspace{-1.5em} % Adjust the vertical spacing as needed

    \label{fig:icn_ll_scaling}
\end{figure}

==> Figures/Tex/MEMBW_scaling.tex <==
\begin{figure}[b!]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=25em]{Figures/Sources/MemBW_scaling_prefill.pdf}
        % \vspace{-1em}
        \text{(a) Prefill \xbox}
        \label{fig:MemBW_scaling_prefill}
    \end{subfigure}
    
    % \vspace{1em} % Adjust the vertical spacing as needed
    
    \begin{subfigure}
        \centering
        \includegraphics[width=25em]{Figures/Sources/MemBW_scaling_decode.pdf}
        % \vspace{-1em}
        \text{(b) Decode \checkbox} 
        \label{fig:MemBW_scaling_decode}
    \end{subfigure}
    
    % \vspace{1em} % Adjust the vertical spacing as needed
    \vspace{-0.5em} % Adjust the vertical spacing as needed

    \caption{Scaling Memory bandwidth per accelerator for text summarization use case.  Mixtral requires only 2 accelerators. GPT3 uses 12 accelerators with TP:12.}
    \vspace{-1em}
    \label{fig:MEMBW_scaling}
\end{figure}

==> Figures/Tex/Model_arch_compute_vs_memory.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures//Sources/compute_vs_memory_for_model_arch.pdf}
    \caption{Compute FLOPs vs Memory footprint across model architectures. We plot various models of different size for each model architecture. The plot also shows how the requirement changes as context length goes from 1K (Smaller points) to 128K (Larger points). }
    \label{fig:model_arch_compute_vs_memory}
\end{figure}

==> Figures/Tex/Single_Input_Batching.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.90\linewidth]{Figures//Sources/basic_batch_scaling.pdf}
    \vspace{-1em}
    \caption{Impact of batching on decode throughput and TPOT.
    % \GJ{You can put more annotations for B=10, B=20, ..?
    % }
    }
    \vspace{-1em}
    \label{fig:single_input_batching}
\end{figure}


==> Figures/Tex/memory_size_req.tex <==

% [!htbp]
%     \centering
%     \includegraphics[width=1\linewidth]{Figures/Sources/memory_capacity_req_decode.pdf}
%     \caption{Memory Capacity (GB) required for various models on different use cases during the decode stage.}
%     \label{fig:memory_cap_req}
% \end{figure}

==> Figures/Tex/transformer_overview.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{Figures/Sources/LLM Arch.drawio.png}
    \vspace{-1em}
    \caption{Typical LLM Model Architecture. Each Layer has multiple parallel heads. For MoE models, there are multiple parallel MLP layers out of which `k' are activated.
    }
    \vspace{-2em}
    \label{fig:transformer_overview}
\end{figure}

==> Sections/00_coverletter.tex <==
\section{\titleRev{Paper updates and common questions}{blond}}
% \begin{enumerate}[leftmargin=0pt]

\circled{1} \textbf{Additional Validation Studies (\RevC{Rev C}, \RevD{Rev D}, \RevE{Rev E}):}  
We have expanded our validation studies, \autoref{subsec:genz_validation} to include \textbf{chunked serving} in addition to \textbf{prefill} and \textbf{decode} and \textbf{new HW architectures}, including AMD GPU, Intel Gaudi2, and SambaNova SN40L.  


\noindent \circled{2} \textbf{Dataflow/NPU Modeling (\RevA{Rev A}, \RevC{Rev C}, \RevD{Rev D}):}
    % 
% The primary focus of this work is not on simulating the microarchitecture of individual NPUs; rather, the
GenZ framework is designed to primarily model the effects of LLM model architectures and optimizations inference at a platform scale that remains microarchitecture-agnostic. Detailed simulators such as Timeloop~\citep{timeloop}, Scale-sim~\citep{scale-sim}, and Maestro~\citep{maestro} excel in modeling the microarchitectural details of NPUs. 
% NPU's microarchitecture details are incorporated as an efficiency factor derived from specific simulators or real hardware.
GenZ can employ these sophisticated simulation tools to obtain more precise performance projections of individual NPUs. 
Please check updated \autoref{fig:platform_overview} and \autoref{sec:HW_acc_charac} for clarification.
% 
We have added a new case study, \autoref{subsec:c4_uarch_casestudy}, to show the impact of different microarchitectures with GenZ using a cycle-accurate simulator for modeling the microarchitecture.

\noindent \circled{3} \textbf{Efficiency Parameter Calculation (\RevA{Rev A}, \RevC{Rev C}, \RevD{Rev D}):} 
For simulated NPUs, we can get efficiency factors from compute simulator depending on the micro-architecture.
For real NPUs (e.g. GPUs), we estimate efficiency for various operator sizes by profiling kernels on actual hardware.
\autoref{subsec:genz_validation} has additional details about calculating efficiency factors and their values used in validation.
% similar to vidur methodology~\citep{agrawal2024vidurlargescalesimulationframework}.
% By executing multiple runs across different kernel configurations, we obtained the average utilization metrics, enabling us to derive a realistic estimation of kernel efficiency for LLM inference workloads.  
%     \item \textbf{Efficiency Parameter Calculation (\RevA{Rev A}, \RevD{Rev D}):}


\noindent \circled{4} \textbf{Power/Energy Estimations (\RevA{Rev A}, \RevC{Rev C}, \RevD{Rev D}):}  
Case study, \autoref{subsec:c2_arch_comparision}, is updated to incorporate energy estimates across different hardware platforms. As suggested by reviewers, energy calculations consider the utilization of individual platform components.
% , following methodologies such as AccelWatch~\citep{AccelWattch}.

\noindent \circled{5} \textbf{Insights Generated from \tool (\RevB{Rev B}, \RevE{Rev E}):}  
Sections 4–6 present insights derived from design exploration experimental studies using \toolns. \autoref{sec:platform_impact} presents detailed case studies at the platform level with insights in designing next generation platforms.  \autoref{subsec:c2_arch_comparision} highlights performance trade-offs across different workloads, demonstrating that certain architectures are more suited for specific tasks.
% \end{enumerate}
\vspace{-1em}
\section{Addressing specific questions}

\subsection{\titleRev{Reviewer A clarifications}{colorRevA}}

% \begin{enumerate}
\noindent \circled{1} \textbf{Power Clarification:} 
The power values (57.2kW) presented in Section 6.2 correspond to 4x B200 rack (14.3kW). 
% The revised version of the paper provides additional clarification on this matter.  

\noindent \circled{2} \textbf{SambaNova vs. GPUs:} 
We acknowledge the architectural differences between SambaNova NPUs and GPUs, but they share fundamental structural similarities, each comprising dedicated compute resources, local SRAM, and HBM/DRAM for memory access.
% 
% Other accelerators, such as TPUs, also fall within this broader category.
The configuration in \autoref{subsec:c2_arch_comparision} corresponds to a B200 configuration.
% 
Our modeling approach remains microarchitecture-agnostic, enabling us to categorize these architectures under a unified framework.  
% \end{enumerate}

\noindent \circled{3} Text added in \autoref{sec:llm_optimization_impact}  as suggested and Etched link fixed. 

\vspace{-1em}

\subsection{\titleRev{Reviewer B clarifications}{colorRevB}}
% \begin{enumerate}
\noindent \circled{1} \textbf{Distinction from a Simple Roofline Model: }
GenZ extends beyond a conventional roofline model by providing a comprehensive framework for architectural design exploration in LLM deployments. Unlike basic roofline analysis tools (e.g., LLMViewer), GenZ incorporates multiple fidelity levels, accounting for model architecture, software optimizations, and hardware-specific tuning, thereby enabling a more holistic design space exploration.  

\noindent \circled{2} \textbf{GenZ as an API:} 
\tool is implemented as a robust and modular Python library and can be installed as a pip package. Users can seamlessly install and do API calls on CPU-based systems with minimal setup overhead.  

\noindent \circled{3} \textbf{Need for Distributed Cluster Modeling:} 
Given the increasing adoption of distributed clusters for LLM inference, it is imperative to model NPUs interconnected through hierarchical, multi-dimensional topologies. GenZ provides insights into the design and performance trade-offs of such distributed systems.  


% \end{enumerate}
\vspace{-1em}
\subsection{\titleRev{Reviewer C clarifications}{colorRevC}}
% \begin{enumerate}

\noindent \circled{1} \textbf{Offloading Modeling:} 
GenZ currently models memory storage offloading, wherein a portion of model weights and KV cache can be offloaded to remote memory. Compute operations can also be offloaded based on workload requirements. \autoref{subsec:c4_uarch_casestudy} shows a case with some operators being offloaded to a CPU.

\noindent \circled{2} \textbf{Interconnect Non-Determinism:} 
As correctly noted, large-scale simulations introduce non-deterministic communication delays due to network contention. In GenZ, ASTRA-Sim is responsible for modeling network traffic dynamics. Users can configure the simulation fidelity to be either congestion-aware or congestion-unaware. In both cases, the framework ensures that collective operations complete before subsequent kernel execution proceeds.  

\noindent \circled{3} \textbf{Data Distribution in Heterogeneous Networks:} 
For mix of high and low speed ICNs, workload distribution strategies can vary. GenZ assumes homogeneous workload distribution among nodes with similar interconnect levels. \tool can explore different parallelism mapping across the physical and logical levels. 

\noindent \circled{4} \textbf{Heterogeneous Modeling:} 
\tool supports network heterogeneity by allowing for different interconnection schemes as described in Section 6.3. \tool currently assumes uniform NPU configurations to avoid complexities arising from imbalanced workload distribution and additional parallelism strategies.

\noindent \circled{5} \textbf{GenZ Performance:} 
GenZ processes around 100 data points per minute on a 32-core x86 CPU. There would be some potential slowdowns based on the fidelity of NPU or network simulators.

 
% \end{enumerate}
\vspace{-1em}

\subsection{\titleRev{Reviewer D clarifications}{colorRevD}}
% \begin{enumerate}
    % \item Table 5 has been updated to provide detailed platform parameters.  
    % \item Efficiency factor calculation details are included in the common section.  
    % \item Additional architectural validation has been conducted within GenZ.  
% \noindent \textbf{Architecture parameters}: For each architecture in \autoref{tab:platform_arch}, PFLOPs column show
\noindent \circled{1} \textbf{\autoref{tab:platform_arch}}: Please review updated table and caption.

\noindent \circled{2} \textbf{Disaggregated serving} requires cluster-level modeling, where dynamic scheduling delays influence request latency. Since \tool alone cannot capture this behavior, we are developing a secondary scheduler to integrate with GenZ, enabling asynchronous request handling across machines as a future work.

\noindent \circled{3} \textbf{Sections 4.3 and 5} highlight GenZ’s ability to support researchers without specialized hardware and provide a predictive framework for evaluating future models and systems before deployment, with H100x8 modeling as an example.
  
\noindent \circled{4} \textbf{Why was expert-parallelism not used in MoE in Section 6.3?}  While expert-parallelism is an important consideration for MoE models, we find that HBD is critical for optimizing tensor-parallel workloads, which aligns with current best practices and thus EP was not considered for this case study.
% \end{enumerate}
% \subsection{\RevE{Reviewer E} clarifications}
% % \begin{enumerate}
% \noindent \textbf{Additional Validation: }
% As noted previously, we have expanded our validation studies to include additional optimizations and diverse hardware platforms. Figure 5 presents validation results for both the prefill stage (left: TTFT) and the decode stage (right: throughput) across multiple LLM architectures and hardware configurations.  

% \textbf{Paper Organization and GenZ Optimizations:}
% Following the reviewer’s suggestion, the paper structure has been revised:  
% - Section 3 describes the components of GenZ along with relevant validation studies.  
% - Sections 4–6 present insights derived from experimental studies using GenZ.  
% All optimizations and model architectures discussed in Sections 4–6 are implemented within the GenZ framework.  

% \end{enumerate}





==> Sections/01_intro.tex <==
\section{Introduction}
\label{sec:intro}
% Generative AI has become an integral part of our daily lives, playing a crucial role in a wide range of everyday applications. These powerful models have grown extensively in popularity and utility, revolutionizing the way we interact with technology and access information. From voice assistants like Siri and Alexa that help us with tasks and answer questions, to recommendation systems on platforms like Netflix and Amazon that personalize our content, Generative AI models are behind the scenes, shaping our digital experiences. Furthermore, their uses continue to expand into new domains, including healthcare, finance, and education, demonstrating their versatility and potential for transformative impact. Additionally, generative AI’s impact on productivity could add trillions of dollars in value to the global economy. It is estimated that gen AI could add the equivalent of 4.4 trillion annually, which would larger than world's 3rd largest GDP~\cite{McKinseyReport}.
Large language models (LLMs) are among the most popular variants of generative AI models performing auto-regressive tasks. LLMs are used in various applications, including chatbots, code generation, question answering, chemical property prediction ~\cite{CHEMBERT}, protein sequencing ~\cite{Brandes2022}, and video generation ~\cite{kondratyuk2024videopoet, oaisora}.
% 
Commercial products like ChatGPT, Gemini, Github Copilot ~\cite{chatgpt, Gemini, copilot}, have performed astonishingly well in diverse metrics, often outperforming human experts ~\cite{LLMIQ}. 
% 
LLMs have shown great scaling law property ~\cite{kaplan2020scaling, caballero2023broken}, with larger models ~\cite{GPT3, claude, chowdhery2022palm} demonstrating better performance as compared to the smaller ones ~\cite{wei2022emergent}. 
% 
% \autoref{fig:model_trends} shows the how LLM models have out grown the hardware memory size growth. 
Currently, the largest model has $\sim$1.8T parameters ~\cite{informationisbeautiful}, and future LLMs potentially would have even a few hundred trillion parameters. 
% 
%Distributed LLM serving is the only way to enable serving these models to meet the large capacity requirement.
% 
To serve those parameter-heavy LLM models effectively, \textit{distributed hardware platforms}\footnote{We define platform as the complete hardware back-end including multiple NPUs (e.g., GPUs or TPUs), local memories (e.g. HBM) and inter-NPU interconnect (e.g., NVlinks/XeLinks).} with enormous compute power and memory resources is necessary. 

% Simultaneously, reducing latency and improving throughput are critical to maintaining cost-effective inference services. \textit{Thus, the systems for LLM inference services should possess parallel processing capabilities, high-speed storage solutions, and highly scalable networks.}


% LLM training has been a focus of research since introduction of LLMs. The challenge revolving LLM training are also being solved by scaling up the compute per hardware. Works like ~\cite{} have helped achieve near linear  with more node.
LLM inference can be broken into two stages, namely the \textit{prefill} and the \textit{decode} stage. The prefill stage consists of a single forward pass using all the input tokens. The auto-regressive decode stage generates one output token with each forward pass of the model. The prefill stage often portrays characteristics similar to training forward pass and has significant computing requirements. In contrast, the decode stage requires high memory bandwidth (BW) and capacity (especially when processing long context queries). 
%\autoref{fig:various_stage_HW_req} portrays the contrast in hardware requirements at different stages in the LLM life-cycle, namely, LLM training, inference-prefill and inference-decode stage.
%\TK{I think you should mention this is summary from from our analysis in paper.}
%\GJ{I think it would be good to use a concrete example with the actual numbers.}

To provide efficient LLM inference, extensive efforts are being made to develop optimizations from both the industry and academic community, including model compression (quantization ~\cite{gholami2022survey, kang2024gear, xiao2023smoothquant}, pruning ~\cite{frantar2023sparsegpt,  bambhaniya2024progressive, jeong2024abstracting},
% knowledge distillation~\cite{gou2021knowledge,hinton2015distilling}), 
fast token decoding ~\cite{kim2024speculative,fu2024break, elbayad2019depth,chen2023ee}), system optimizations (paged attention ~\cite{kwon2023efficient}, flash attention ~\cite{dao2022flashattention}, chunked inference ~\cite{holmes2024deepspeed, agrawal2023sarathi}, scheduling ~\cite{yu2022orca}), and so on. 
Many of these techniques have also become part of the popular inference-serving engine 
% \TK{@Abhi you had called them inference engines and inference servers - i wasnt sure what the difference is so merged them into one category called inference serving frameworks }
such as TensorRT-LLM ~\cite{TensorRT-LLM}, vLLM ~\cite{kwon2023efficient}, and DeepSpeed-FastGen ~\cite{holmes2024deepspeed}.
% and inference servers such as 
% RayLLM ~\cite{ray-llm} with RayServe, TGI~\cite{tgi} and TensorRT-LLM + Triton~\cite{triton}.

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{Figures//Sources/model_vs_HW_size.png}
%     \caption{Frontier generative models memory size (Red) compared to latest generation inference hardware memory capacity(Blue). Model size have outpaced hardware memory size by 300x, generating the need for distributed inference. }
%     \label{fig:model_trends}
% \end{figure}

\begin{figure}[!pt]
    \centering
    \includegraphics[width=\linewidth]{Figures/Sources/Platform_req_sypder.pdf}
    \vspace{-2em}
    \caption{Platform requirements for two workloads.}
    \label{fig:various_stage_HW_req}
    \vspace{-1em}
\end{figure}
%are examples that try to achieve optimized inference performance for a hardware platform \footnote{Platform is defined as the complete hardware back-end. (Multiple Accelerators connected in a particular fashion)}. Additional optimizations including .
% \AB{@TK: Can you iterate here?}
% \SK {The contribution part if more clarified would be better, currently it is written like only insights, do you want to have the GenZ as your contribution as well? if so, please have 1. a framework/analyzer as the first, 2. insights as the second, and then elaborate briefly on it. Also, they are discretely placed, please consolidate the contributions.}
% \AB{This is a positioning thing i feel. We are definitely going to open-source the tool that to this week. For the micro, i was consciously try to stay away from saying tool, because than they want extensive validation. Personally, I feel the tool is a \textbf{valuable} contribution, however so are the insights. @SK , @TK what do you suggest?}\TK{A bulk of paper is Section III so it should be a contribution. And whether or not you call it as a contribution, ppl will ask for validaiton of methodology. So it should be a contribution. You can call it a ``first-order model" for architectural insights. You are not claiming cycle accuracy or anythingoh t}
\input{Tables/Releated_Work_comparsion}

\input{Figures/Tex/gen_overview_figure}

The aforementioned works have enabled vast inference performance improvements for LLMs on current hardware platforms.
% 
Unfortunately, they do not automatically provide an answer to how to design \textit{next-generation platforms} for LLM inference due to an extremely large and inter-dependent design space on the workload side spanning a large plethora of emerging LLMs with increasing accuracy and context lengths ~\cite{zhao2023survey}, a diverse suite of LLM inference use cases (such as chatbots, code generation, question answering, chemical property prediction ~\cite{CHEMBERT}, protein sequencing ~\cite{Brandes2022}, and video generation ~\cite{oaisora, kondratyuk2024videopoet}), model-level optimizations (such as quantization, sparsity, kernel fusion, early exit) and system-level optimizations (such as batching, parallelism, chunked prefill, speculative decoding). There also exist several LLM serving platform vendors (such as NVIDIA~\cite{nvidia_hopper}, Intel~\cite{intel_gaudi}, AMD~\cite{AMDMI325X}, Google~\cite{tpu_pods}, Cerebras~\cite{cerebras}, Groq~\cite{Groq}, Sambanova~\cite{sambanova} and others~\cite{amazon_ec2, HotChips65:online}), with distinct choices for HW (compute, memory and network fabrics), managed via custom (often proprietary) SW frameworks.
The combination of these makes it extremely challenging to identify the technology targets (such as compute FLOPs, memory capacity, memory bandwidth, link latency, link bandwidth) and corresponding architectural choices to scale (such as scale-up + scale-out network hierarchy, HBM + DRAM-offload-based memory hierarchy and waferscale) when designing next-generation LLM serving platforms.


%each claiming their specific HW + SW solution is the most optimal. 
% However, as computer architects, we would like to understand the hardware requirements to build \textit{next-generation platforms} for LLM inference.
%This remains an open and challenging question to answer given a diverse suite of LLM inference use cases, a plethora of emerging LLMs with increasing accuracy and context lengths~~\cite{zhao2023survey, }\footnote{In fact on April 18 2024, the day of MICRO's  submission deadline, Meta launched LLaMA3~~\cite{llama3}, which we were able to include in our evaluations (demonstrating the agility of our analysis framework). In March 2024 itself, several startups including Mixtral~~\cite{jiang2024mixtral}, xAI~~\cite{grok}, Databricks~~\cite{dbrx} and SambaNova~~\cite{sambanova} released open-source LLMs. We include Mixtral's 8x7B in our evaluations. This trend make the analysis in this work extremely timely}, and several AI platform vendors (e.g., NVIDIA, Intel, AMD, Google, Cerebras, and others) each claiming their specific HW + SW solution is the most optimal. 




% As LLMs grow larger, analyzing the inference performance on distributed platforms is very critical. 
% % \TK{@Abhi - i made some edits to the following lines}
% The choices of both model-level (e.g., quantization, sparsity, kernel fusion, early exit) and system-level optimizations (e.g., batching, parallelism, chunked prefill, speculative decoding) are important design aspects that must be explored for an efficient LLM serving platform. However, only a subset of these choices can be modeled by simulation frameworks today, leaving more efficient architectures unexplored. 
% 
As computer architects, we look to modeling tools to navigate design-spaces. Today, there exist several open-source modeling tools
for designing optimized accelerators 
~\cite{scale-sim,timeloop,maestro}, 
but none of them provides support for distributed platforms.
%Current simulation frameworks fall short in this aspect as they are unable to simulate distributed platform and provide insights which can help in optimizing the end to end LLM inference performance.
% 
%The choices of batching, parallelism, quantization are important design aspects that need to be explored in combination for an efficient LLM serving. However, only a subset of these choice can be modelled by existing frameworks,
%leaving more efficient designs unexplored. 
Existing frameworks ~\cite{cho2024llmservingsimhwswcosimulationinfrastructure, astrasim, zhang2023hardware} to simulate LLM performances on distributed platforms generally are over-fitted on that of dense transformers. This essentially makes such simulators fall short in terms of capturing the state-of-the-art (SOTA) model architectures beyond traditional transformers. Additionally, these tools~\cite{agrawal2024vidurlargescalesimulationframework, yuan2024llm} only capture a small subset of model \& system optimizations as well as platform architecture choices (refer to \autoref{tab:related_works}), limiting their wide-spread adaptation.


%% Move these specifics to related works.
% there is a lack of support for modeling architectures other than dense transformer. In fact most of the current framework cannot support latest generation SOTA models like Meta's Llama-3~\cite{llama3, dubey2024llama3herdmodels}, Google's Gemma2~\cite{gemmateam2024gemma2improvingopen}, Alibaba's Qwen2.5~\cite{qwen2.5, qwen2, hui2024qwen25codertechnicalreport}, Microsoft's Phi3~\cite{abdin2024phi3technicalreporthighly}, MistralAI's mixtral/mistral~\cite{jiang2023mistral7b, jiang2024mixtral, mixtral22b, }, Nvidia's Nemotron models~\cite{nvidia2024nemotron4340btechnicalreport, parmar2024nemotron415btechnicalreport}.
% % 
% While a plethora of software optimization techniques are available in the open-source community, current frameworks can't model most of these effect of these techniques. Flash-attention, fixed precision quantization are implemented in LLM-viewer and LLMServingSim.
% % 
% % Vidur supports
% % 
% For modeling distributed AI serving platforms, newer models require larger multi-dimension nodes ~\cite{NVIDIABlackwellBox}, none of the current frameworks can do multi-dimensional network modeling for diverse AI platform architectures.


% highlight key aspects where existing distributed ML system modeling frameworks are lacking in \autoref{tab:related_works}.
% 
We aim to demystify and quantify AI platform design insights across a suite of LLM model architectures, inference optimizations, and use cases.
% 
% platforms and  platforms can help us 
% To better understand the problem space, we provide details about the requirements for various LLM platform characteristics in two distinct phases.
% \textbf{LLM serving platforms are used based on empirical insights}. 
% 
% We employ first-order equation-based analysis to 
%
To this end, we introduce a \textit{first-order} analytical model, namely \tool (\underline{Gen}erative LLM analy\underline{Z}er). It distills the complex interplay between model architecture, inference optimizations, and hardware configurations to narrate the end-to-end LLM inference performance. 
% 
\textit{It should be noted that \tool does not not intend to simulate individual NPUs, rather we focus on simulating the distributed platforms for various LLM architectures combined with inference optimizations.}
% 
% %Today, there exist several open-source modeling tools
% for designing optimized accelerators  While tools like timeloop~\cite{parashar2019timeloop} and scale-sim~\cite{scale-sim} can do a very good job at simulating individual accelerators, \tool is meant to simulate a generic NPU. 
% 
% For more detailed simulation of particular accelerator, \tool can use the time generated by these sophisticated tools.
% 
%Before using \tool for experiments, 
We validate \tool thoroughly with various LLMs served across different platforms. Interestingly, across different workloads, \tool can closely mimic the performance on real systems, achieving a {geomean error of only 2.73\%}.
% We can use \tool to study current generation platforms via efficiency factors for the hardware components (which we determine from real-system validation measurements) without getting limited by their specific software toolchains. 
% 
% We use \tool to quantify the hardware requirements for different LLM use cases.
% 
% These studies help us gain first-order vendor-agnostic insights into platform design and configurations.
% \footnote{On April 18th, 2024, the day of MICRO's submission deadline, Meta launched LLaMA 3~~\cite{llama3}
% We include the result with LLaMA 3 in our evaluation to highlight how agile our analysis framework is. 
%In March 2024 itself, several startups including Mixtral~~\cite{jiang2024mixtral}, xAI~~\cite{grok}, Databricks~~\cite{dbrx} and SambaNova~~\cite{sambanova} released open-source LLMs. We include Mixtral's 8x7B in our evaluations. This trend make the analysis in this work extremely timely
% }.

%There have been several articles studying the performance of different LLM models and optimizations on existing real systems. 
%\TK{the next line should be made more precise/stronger}
%To the best of our knowledge, this is the first work to provide platform-level insights for a suite of LLM models serving on different use cases.
% To the best of our knowledge, this is the first work to quantify platform scale requirements for serving future generative AI models for different use cases.
% 
% We believe this work makes three key contributions to the community. First, 
% The analysis presented can potentially guide AI engineers working on LLM deployment to choose suitable hardware platform configurations for their use case(s). 
%For instance, 
% 
%In specific, this work can help answer various system-level choice-making questions, including,  
%(i) how should the deployment platform change for LLM use cases for Q/A chatbots for customer services agents versus legal document summarization in attorney's offices? (ii) how can the platform configurations be tweaked to maintain the same level of performance when deploying LLaMA2-70B instead of LLaMA2-7B? (iii) What will be the performance compromise if we do not change the serving platform?
The analysis presented in this work can provide concrete directions to computer architects designing the next generation AI platforms.
%based on models and compute demand. 
%When building a future system, there are various uncertainties around the interplay between various hardware characteristics and LLM inference performance.
%For instance, if each node's total HBM bandwidth increases/decreases by 10\%, what would the impact on inference latency be? By how much should the chip-to-chip communication network be improved? 
%(iii) Finally, the ultimate question that several computer architects would like to answer: what theoretical hardware configurations are required to build a platform enabling real-time conversation with an AI agent?
%\footnote{Such as J.A.R.V.I.S. in Marvel Cinematic Universe.}? 
%(i) how should we partition the pins of the next NPU between memory versus inter-NPU interconnect? (ii) should we provide high-capacity HBMs per NPU or cheaper low-capacity HBMs and rely on offload to CPU memory, (iii) should we build one datacenter platform for all LLM inference use cases or build different skus?
% 
% \textbf{When building a future system, there are various uncertainties around the interplay between various hardware characteristics and LLM inference performance}. This work can address open questions, such as i.) If each node's total HBM bandwidth increases/decreases by 10\%,
% % 
% what would the impact on inference latency be? ii.) How much should the chip-to-chip communication network be improved? Finally, the ultimate question that every computer architect would like to answer is \textbf{what theoretical system could support Super-LLMs?} What theoretical parameters are required to build a platform enabling real-time conversation with super LLM?  
%
%\TK{I added this line - we should finalie once the new spider plots added}
For instance, \autoref{fig:various_stage_HW_req} highlights a subset of our key observations for two distinct deployment scenarios.
% 
We have quantified and noticed a significant difference in the serving requirements between the prefill and decode stages. Despite the fluctuation of absolute values with the workload, the identified trend remains consistent.
% 
For example, we identify FLOPS and interconnect bandwidth as the bottleneck during the prefill stage, while memory bandwidth and interconnect link latency remain key bottlenecks during the decode stage.

% \TK{@Abhi - pls add 2-3 lines once the new spider plots added}




To summarize, this work makes the following contributions: 
% \begin{itemize}[leftmargin=0pt]

\circled{1}  We introduce \toolns, an analytical framework that helps analyze LLMs combined with various inference optimizations on different platforms (\autoref{sec:methodology}). \autoref{fig:platform_overview}(a) shows an overview of our proposed framework.

\circled{2}  Using \toolns, we study the impact of various LLM serving optimizations with current hardware specifications, and present key insights to guide the next-generation design specifications (\autoref{sec:llm_optimization_impact}).

% $\bullet$  We present detailed runtime analysis across various LLM architectures based on both the transformer and state-space models (\autoref{sec:model_arch_impact}).

    %\item We showcase three key case studies regarding next-generation AI inference platform design:
    %\begin{enumerate}
    %    \item Scaling different platform characteristics independently(\autoref{subsec:scaling_platform}).
    %    \item Comparing different AI platform architecture design choices (Eg, SRAM-Chiplet, Wafer-scale, GPUs, ASICs) (\autoref{subsec:c2_arch_comparision}).
        % for serving LLMs.
    %    \item Studying choice of design space of high bandwidth domain size and different interconnects (\autoref{subsec:c3_network_comparision}).
    %\end{enumerate}
    % \item We analyze the performance impact of different platform characteristics using \toolns.   
    %\autoref{sec:platform_impact}: Trends and insights pertaining to different platform configurations.
    % \item We analyze the platform requirements for the target LLM inference to meet the given SLOs with the target use case using \toolns.
    %\autoref{sec:platform_requirements}: We quantify the platform requirements to support different LLMS for various use cases.
    %\item \autoref{sec:Extreme_scale}: Comparing requirements for future LLM model and perspective of the state of current systems.
% \end{itemize}

% \noindent
\circled{3} Lastly, we showcase \toolns's modeling capability through four case studies on the next-generation AI inference platform design: (1) isolated scaling of different platform characteristics (\autoref{subsec:scaling_platform});
(2) comparison of different AI platform architecture design choices (for example, SRAM-Chiplet, Wafer-Scale, GPUs, ASICs) (\autoref{subsec:c2_arch_comparision}); (3) study design space choices of high bandwidth domain (HBD) size as well as associated interconnects (\autoref{subsec:c3_network_comparision}); and (4) study the impact of micro-architecture details and compute offloading(\autoref{subsec:c4_uarch_casestudy}).

%\GJ{Missing Related works and Conclusion?}
%\TK{for a paper like this which is purely on analysis, it actually helps if the end of the intro summarizes some of our key findings/insights. Maybe this is the right place to refer to Figure 1 as well}
% 
% \section{Key Takeaways}
% Following are the key takeaways from our work. For detailed understanding please read the rest of the paper. You can also use our code to regenerate the results.
% \label{sec:takeaways}
% \begin{itemize}
%     \item The prefill and decode stages of the LLM inference process have significant differences in their workloads. 
%     \item We find that \textbf{increasing} the TFLOPS and inter-chip bandwidth reduces the \textbf{prefill} latency however doesn't impact the decoding latency.
%     \item On the other hand, \textbf{increasing} the high-speed memory bandwidth(HBM) and reducing the inter-chip network link latency helps improve the latency of the \textbf{decode} stage however does not reduce the latency of the prefill stage.
%     \item We also find that for larger systems parallelism plays a major role, where in the \textbf{prefill} stage, using\textbf{ pipeline parallelism} gives the best throughput. During the \textbf{decode} stage, a mix of tensor and pipeline parallelism is optimal for throughput in large systems and \textbf{tensor parallel} for smaller systems. .
%     \item We also quantify the requirements for meeting the SLO throughput requirements of various models with various use cases and provide analytical formulas to modify the demand according to the usecase and model changes. 
% \end{itemize}

==> Sections/05_0_IMpact_model_arch_new.tex <==
\section{Impact of Model Architectures on HW Scaling}
\label{sec:model_arch_impact}

%LLM architectures crucially affect computational efficiency, scalability, and inference characteristics. 

LLM Model architectures are evolving to optimize memory usage, computational cost, and performance across diverse tasks. We compare four state‐of‐the‐art open-source models:
\input{Figures/Tex/Model_Arch_TTFT_TPOT}

\noindent \textbf{Traditional Transformers (Dense):}
Foundational models like Transformer\cite{vaswani2017attention}, GPT, and BERT use fully connected attention, where every token attends to all others. This results in quadratically scaling compute and memory with sequence length.

\noindent \textbf{Dense Transformers with Group-Query Attention:}
\cite{hudson2019gqa} reduces memory costs by sharing key-value caches across heads, improving attention sparsity and overall efficiency for long-context tasks.

\noindent \textbf{Mixture of Experts (MoE):}
MoE architectures leverage sparsity by activating only a subset of expert sub-networks per token, thereby potentially reducing computational load.

\noindent \textbf{Mamba:}
Combining attention mechanisms with RNN-inspired operations, Mamba~\cite{gu2024mambalineartimesequencemodeling} optimizes memory and compute, making it highly effective in large-scale deployments.

For our analysis, we compare models of similar sizes—LLama2-7B\cite{touvron2023llama2}, LLama-3.1-8B\cite{llama3}, Mixtral-8x7B (12.8 Active)\cite{jiang2024mixtral}, and Falcon-Mamba-7B\cite{zuo2024falconmambacompetitiveattentionfree}—by examining how increasing context length and batch size affect latency across different inference stages.

\textbf{1. Impact on Prefill Stage.} \textit{Context Length:}(\autoref{fig:model_arch_impact}(a))
All models show linear latency growth with longer contexts. Notably, even with a constant cache, the Mamba model incurs a linear-time initial scan. With tailored scan kernels, this growth could be reduced to sub-linear levels\cite{gu2024mambalineartimesequencemodeling}.
\textit{Batch Size:}(\autoref{fig:model_arch_impact}(b))
Latency increases linearly across architectures. Dense, Dense-GQA, and MoE models exhibit more efficient scaling, and while Dense-GQA uses fewer KV heads, its performance remains compute-bound.

\textbf{2. Impact on Decode Stage.}
\textit{Context Length:}(\autoref{fig:model_arch_impact}(c))
Mamba maintains constant runtime due to context-length independence, while Dense models suffer significant latency increases due to quadratic attention costs. Dense-GQA and MoE mitigate this effect with smaller KV cache growth.
\textit{Batch Size:}(\autoref{fig:model_arch_impact}(d))
All models display near-linear latency growth; however, the Dense model’s slope is steeper due to larger KV caches, whereas Dense-GQA, Mamba, and MoE benefit from batching to improve throughput.

\textbf{3. Impact on Chunked Stage.}
\textit{Context Length:}(\autoref{fig:model_arch_impact}(e))
In chunked prefill (processing a fixed 512-token chunk), latency scales linearly as larger contexts increase the KV cache size, echoing trends seen in the decode stage.
\textit{Batch Size:}(\autoref{fig:model_arch_impact}(f))
Dense-GQA and MoE show a lower growth rate owing to fewer KV heads. Interestingly, MoE experiences higher latency in the prefill segment because all experts are activated, increasing the overall cost.

==> Sections/91_extra_validation.tex <==
\section{Additional Validation Data}


This section has added details about the data from studies presented in section 3.5. We also have additional studies comparing the collective times with different platform sizes to validate the platform interconnect modeling.

% We study the trends of prefill and decode on different platform systems to validate the accelerator modeling by \toolns. 
% We conduct two types of studies: (i) Trends of prefill and decode on different platform systems to validate the accelerator modeling by \toolns. (ii) Collective times with different platform sizes to validate the platform interconnect modeling.

\subsection{Platform interconnect validation}

We validate the collective time modeled by \tool against real hardware collective values. We use the HGX\cite{nvidia_hgx} box with 8 NVIDIA H100 SXM GPUs (80 GB) fully connected by NVLinks for this experiment.

To verify the collectives time at the platform scale, we benchmark all-reduce communication primitive with nccl-tests\cite{nccl}, a communication primitive performance benchmark for NVIDIA GPUs. 
% 
\tool's collective communication times are validated with a platform size of 2 GPUs, 4 GPUs, and 8 GPUs.
% 
For collective communications, we observed an average link efficiency of 75\% for NVLINK, which gives an effective link BW of 350 GB/s for each GPU in HGX box.
% 
We profile all combinations of use case (Table 3) and model (Table 2) and collect their all-reduce (AR) message sizes. 
% 
The message size of each AR call is very small ($<$ 128 KB) for decode, while for prefill, per call message size is a few hundred MBs.
% 
\autoref{fig:AR_validation.} compares the real hardware latency for three different platform sizes and the corresponding latency generated by \tool.
% 
Since the prefill and decode stages have stark differences in message size, we verify the collective time for prefill and decode independently.
% 
We found that for decode message sizes, the link latency, $T_{Link}$ is the dominating, thus the latency seems almost constant.
% 
While prefill AR messages are large enough, the link bandwidth, $BW_{Link}$, is the main contributor to collective time.
% 
Collective for all datapoints, there is a 3.89\% and 2.7\% geomean error for decoding and prefilling message sizes between real values and \tool values.



\begin{figure}[!b]
    \centering
        % \hfill
    \begin{subfigure}
        \centering
        \includegraphics[width=11.5em]{Figures/Sources/AR_prefill_validation.pdf}
        % \caption{Prefill Message size}
        \label{fig:ar_prefill_validation}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=11.5em]{Figures/Sources/AR_decode_validation.pdf}
        % \caption{Decode Message sizes}
        \label{fig:ar_decode_validation}
    \end{subfigure}
% \vspace{-1em}
    \caption{Comparing All Reduce NCCL latency from \tool against HGX:8xH100 box. Platform sizes of 2, 4, and 8 GPUs for varying message sizes.}
    % \vspace{-1em}
    \label{fig:AR_validation.}
\end{figure}

\subsection{NPU validation data}

\autoref{tab:all_validation} shows the error between real value and \tool predicted value for each hardware platform.
The prefill error column represents an error in TTFT calculation. Similarly, the decode error column represents the error in the decode throughput calculation.
Each value in the table is the geomean error for all the data points of the given hardware platform.

\input{Tables/all_validation_error}

==> Sections/92_All_scaling.tex <==
\section{Platform Characteristics Analysis: Additional data}

This section shows the data for all LLM models for all usecase from section 5.

For all studies we keep the baseline NPU  with 800 TFLOPS, 40 GB HBM memory @ 4000 GB/s memory bandwidth,  300 GB/s interconnect bandwidth, and link latency of 2 us.

We explore four key platform characteristics: TFLOPS ($HW_c$), Memory BW ($BW_{fast}$), ICN link bandwidth ($BW_{link}$), ICN link latency ($T_{Link}$)

We show the scaling of each individual platform characteristic for various different models and all 5 use cases as show in Table 3 of the main paper.

% \subsection{TFLOPS Scaling}

\begin{figure*}[h]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=50em]{Figures/Sources/TFLOPS_scaling_all_prefill.pdf}
        % \vspace{-2em}
        \text{(a) Prefill \checkbox}
        % \label{fig:TFLOPS_scaling_prefill}
    \end{subfigure}
    
     % \vspace{-0em} % Adjust the vertical spacing as needed
    
    \begin{subfigure}
        \centering
        \includegraphics[width=50em]{Figures/Sources/TFLOPS_scaling_all_decode.pdf}
        % \vspace{-2em}
        \text{(b) Decode \xbox}
        % \label{fig:TFLOPS_scaling_decode}
    \end{subfigure}
    
     % \vspace{-0.5em} % Adjust the vertical spacing as needed

    \caption{Scaling TFLOPS for various models all use case. Mixtral requires only 2 accelerators. GPT3 uses 12 accelerators with TP:12.}
    % \vspace{-1em}
    % \label{fig:TFLOPS_Scaling}
\end{figure*}

% \clearpage

% \subsection{Memory Bandwidth Scaling}
\begin{figure*}[h!]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=50em]{Figures/Sources/MemBW_scaling_all_prefill.pdf}
        % \vspace{-1em}
        \text{(a) Prefill \xbox}
        \label{fig:MemBW_scaling_prefill}
    \end{subfigure}
    
    % \vspace{1em} % Adjust the vertical spacing as needed
    
    \begin{subfigure}
        \centering
        \includegraphics[width=50em]{Figures/Sources/MemBW_scaling_all_decode.pdf}
        % \vspace{-1em}
        \text{(b) Decode \checkbox} 
        \label{fig:MemBW_scaling_decode}
    \end{subfigure}
    
    % \vspace{1em} % Adjust the vertical spacing as needed
    % \vspace{-0.5em} % Adjust the vertical spacing as needed

    \caption{Scaling Memory bandwidth per accelerator for various use case.  Mixtral requires only 2 accelerators. GPT3 uses 12 accelerators with TP:12.}
    \vspace{-1em}
    \label{fig:MEMBW_scaling}
\end{figure*}
% \clearpage

% \subsection{ICN Bandwidth Scaling}

\begin{figure*}[h!]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=50em]{Figures/Sources/NOCBW_scaling_all_prefill.pdf}
        % \vspace{-2em}
        \text{(a) Prefill \checkbox}
        \label{fig:nvlink_BW_scaling_prefill}
    \end{subfigure}
    
    % \vspace{1em} % Adjust the vertical spacing as needed
    
    \begin{subfigure}
        \centering
        \includegraphics[width=50em]{Figures/Sources/NOCBW_scaling_all_decode.pdf}
        % \vspace{-2em}
        \text{(b) Decode \xbox}
        \label{fig:nvlink_BW_scaling_decode}
    \end{subfigure}
    
    % \vspace{-0.5em} % Adjust the vertical spacing as needed

    \caption{Scaling interconnect network BW for platform running various use case. GPT3 and GPT4 uses 24(TP:12+PP:2) and 84(TP:21+PP:4) NPUs respectively.}
    % \vspace{-1em}
    \label{fig:icn_bw_scaling}
\end{figure*}

% \clearpage

% \subsection{ICN Link Latency Scaling}

\begin{figure*}[!h]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=50em]{Figures/Sources/nvlink_latency_scaling_all_prefill.pdf}
        % \vspace{-0.5em}
        \text{(a) Prefill \xbox}
        \label{fig:nvlink_latency_scaling_prefill}
    \end{subfigure}
    
    % \vspace{1em} % Adjust the vertical spacing as needed
    
    \begin{subfigure}
        \centering
        \includegraphics[width=50em]{Figures/Sources/nvlink_latency_scaling_all_decode.pdf}
       % \vspace{-2em}
        \text{(b) Decode \checkbox}
        \label{fig:nvlink_latency_scaling_decode}
    \end{subfigure}
    
    % \vspace{1em} % Adjust the vertical spacing as needed
    % \vspace{-0.5em} % Adjust the vertical spacing as needed

    \caption{Scaling Interconnect network link latency for LLMs on all use cases. GPT3 uses 24 NPUs with TP:12+PP:2, and GPT4 uses 84 NPUs with TP:21+PP:4. }
    % \vspace{-1.5em} % Adjust the vertical spacing as needed

    \label{fig:icn_ll_scaling}
\end{figure*}

==> Sections/93_Quantization_scaling.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/Sources/quantization_scaling.pdf}
    % \vspace{-2em}
    \caption{Quantization Scaling }
    % \vspace{-1em}
    \label{fig:memory_cap_req}
\end{figure*}

==> Sections/97_2_Extreme_requirements_prediction.tex <==
\section{Extreme Scale Requirements: Sequence Prediction}
\label{sec:Extreme_scale}

Batch Size = 1
Beam Size = 4
Num Generated tokens = 2000


% \begin{figure}[h]
%     \begin{subfigure}[]{1\textwidth}
%         % \centering
%         \includegraphics[width=0.7\linewidth]{}
%         \caption{Memory Bandwidth (TB/s) }
%         \label{fig:extreme_memory_bw_req}
%     \end{subfigure}
    
%     \vspace{1em} % Adjust the vertical spacing as needed
    
%     \begin{subfigure}[]{1\textwidth}
%        % \centering
%         \includegraphics[width=0.7\linewidth]{}
%         \caption{Memory Capacity (PB).}
%         \label{fig:extreme_memory_cap_req}
%     \end{subfigure}
%     \caption{Platform Scale requirements supporting a real-time  conversational AI personal assistant.}
%     \label{fig:ai_assistant_req}
% \end{figure}

If we make a 10T parameter personalized AI models, which can in real conceptualize one million context length inputs, it would have numerous applications. Virtual Assistants, Personalized Education, Language Translation and Interpretation, Emotional Support and Therapy

In compercial context it can help in Scientific Research: LLMs can assist in literature review, hypothesis generation, experiment design, and data analysis, accelerating scientific discovery and innovation.
Healthcare Applications: LLMs can be used for medical question-answering, diagnostic assistance, treatment recommendation, and even drug discovery by processing vast amounts of medical literature and data.
Cybersecurity: LLMs can be used for threat detection, vulnerability analysis, and even generating secure code or identifying security flaws in existing codebases.
Creative Design: LLMs can assist in generating ideas, concepts, and even detailed designs for products, architecture, fashion, and various creative endeavors.


Key Takeaway :- 



\textbf{Short Context, Short Generation, Low Latency:}
- Customer Service (chatbots, virtual agents)
- Language Translation
- Basic Question-Answering
These applications typically involve short prompts or queries (context) and require generating relatively short responses in real-time or with low latency.


\textbf{Medium Context, Medium Generation, Moderate Latency:}
- Personalized Education
- Intelligent Assistants
- Medical Question-Answering
- Legal Assistance

These applications may involve longer prompts or context (e.g., student's learning history, medical records, legal documents) and require generating moderately lengthy responses, such as explanations, summaries, or recommendations. The expected latency can be moderate, ranging from a few seconds to a few minutes.


\textbf{Long Context, Long Generation, High Latency:}
- Automated Writing (articles, stories, scripts)
- Scientific Research (literature review, hypothesis generation)
- Creative Design


These applications often involve processing and understanding large amounts of context (e.g., research papers, books, design specifications) and generating lengthy and complex outputs, such as articles, stories, research proposals, or design concepts. The expected latency can be higher, ranging from minutes to hours or even days, depending on the complexity of the task.


It's important to note that the categorization is not absolute, and some applications may span multiple categories depending on the specific use case and requirements. Additionally, as LLM technologies continue to advance, the latency expectations and generation capabilities may improve, potentially blurring these boundaries.

### GEMINI
Short Context, Short Generation, Low Latency

Real-time conversation assistants: LLMs can act as conversation partners, providing summaries of factual topics, translating languages on the fly, or generating different creative text formats like poems or code based on short prompts and responding to follow-up questions within the conversation https://aisera.com/chatbots-virtual-assistants-conversational-ai/.
Content moderation: Quickly analyzing short pieces of text or code for harmful content or spam can be done with low latency LLMs trained on large amounts of labeled data.
Smart replies for emails/drafts: LLMs can suggest short, context-appropriate replies to emails or generate different creative text formats based on the content of the email.
Medium Context, Medium Generation, Medium Latency

Automatic summarization: LLMs can take in news articles, research papers, or other lengthy text and provide concise summaries that capture the important points. Latency can range from a few seconds to a few minutes depending on the complexity of the input text.
Machine translation: LLMs can translate between languages while considering the context of the text to provide more accurate and nuanced translations. Latency can vary depending on the length of the text and the target language.
Code generation/completion: LLMs can take a piece of code with missing parts and complete it based on the context or translate natural language instructions into functional code. Latency can vary depending on the complexity of the code.
Long Context, Long Generation, High Latency

Script writing: LLMs can generate scripts for movies, TV shows, or plays based on a story outline or concept, considering character development, plot flow, and dialogue. This can be computationally expensive and take a long time to generate.
Creative writing: LLMs can write different kinds of creative content like poems, code, scripts, musical pieces, email, letters, etc. given a starting prompt or theme. The latency can be high depending on the length and complexity of the desired output.
Research paper generation: LLMs can assist researchers in writing research papers by summarizing existing literature, suggesting citations, and generating different sections of the paper based on provided information. This task can be computationally expensive and take a significant amount of time.
Additional Factors

Task complexity: More complex tasks, such as writing a novel or composing a symphony, will likely require longer context lengths, generation lengths, and higher latency.
Availability of computational resources: The latency of LLM tasks will also depend on the availability of computational resources. As hardware and algorithms improve, LLMs will be able to handle more complex tasks with lower latency.
It's important to note that this is a hypothetical categorization, and the actual capabilities of LLMs will continue to evolve. However, it provides a general framework for understanding how context length, generation length, and latency can impact the types of tasks that LLMs can be used for.

### CHAT GPT
Certainly! Let's categorize the futuristic tasks based on context length, generation length, and output generation latency expectation:

### Context Length:
1. **Short Context**:
   - Virtual Personal Assistants
   - Customer Service and Support
   - Crisis Management and Disaster Response
   - Autonomous Vehicles Interaction

2. **Long Context**:
   - Legal Research and Analysis
   - Medical Diagnostics and Healthcare
   - Financial Analysis and Investment
   - Environmental Monitoring and Conservation

### Generation Length:
1. **Short Generation**:
   - Virtual Personal Assistants
   - Customer Service and Support
   - Crisis Management and Disaster Response
   - Autonomous Vehicles Interaction
   - Language Translation and Interpretation
   - Financial Analysis and Investment

2. **Long Generation**:
   - Content Creation and Generation
   - Historical Reconstruction and Cultural Preservation
   - Space Exploration and Research
   - Ethical Decision-Making and Governance
   - Cybersecurity and Threat Detection

### Output Generation Latency Expectation:
1. **Real-time Response**:
   - Virtual Personal Assistants
   - Customer Service and Support
   - Crisis Management and Disaster Response
   - Autonomous Vehicles Interaction
   - Language Translation and Interpretation

2. **Near Real-time Response**:
   - Medical Diagnostics and Healthcare
   - Financial Analysis and Investment
   - Cybersecurity and Threat Detection

3. **Flexible Response Time**:
   - Legal Research and Analysis
   - Content Creation and Generation
   - Space Exploration and Research
   - Ethical Decision-Making and Governance
   - Environmental Monitoring and Conservation
   - Historical Reconstruction and Cultural Preservation

These categorizations provide insight into the varying requirements and expectations for context length, generation length, and output generation latency across different futuristic tasks enabled by Large Language Models.

==> Sections/99_motivation.tex <==
\begin{comment}
 \section{Motivation}
\label{sec:motivation}

QPS vs Latency

As batch size increases, we can push both prefill and decode into compute-bound regions.

The catch is that this might require a very high batch size to become compute-bound depending on model.

\TODO {FIg1 : For different models, how the KV cache size grows what batch size is required to become compute bounded.[i.e. 128, 256]}

Even you require different beams also.   
\end{comment}


% \subsection{System optimizations}
% We describe different techniques that reduce data movement to improve the model throughput.

% \paragraph{Operator Fusion} Flash Attention/FLAT

% \paragraph{Data Cacheing} KV Cache

% \paragraph{Distributed Inference} Using Multiple devices.

% \subsection{Algorithmic optimizations}
% We describe different techniques that reduce data movement to improve the model throughput.

% \paragraph{Activation Compression} Sparsity and Quantization in KV cache

% \paragraph{Multi Query Attention} MQA , GQA

% \paragraph{Weight Reduction} Sparsity and Quantization.

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{Figures//Sources/Runtime Breakdown.png}
%     \caption{Relative breakdown of critical path in LLMs. \AB{TODO:update data with real data.}}
%     \label{fig:enter-label}
% \end{figure}

==> Tables/all_validation_error.tex <==
\begin{table}[!h]
\begin{tabular}{|c|c|c|}
\hline
Platform & Prefill error & Decode error \\ \hline
2xV100 & 2.40 & 1.41 \\ \hline
2xA100 & 1.98 & 1.48 \\ \hline
1xH100 & 2.72 & 3.02 \\ \hline
2xH100 & 3.73 & 2.02 \\ \hline
4xH100 & 3.94 & 3.10 \\ \hline
8xH100 & 2.18 & 1.02 \\ \hline
\end{tabular}
\caption{Prediction error between \tool and values observed on real hardware system. }
\vspace{-0.5em}
\label{tab:all_validation}
\end{table}

==> Tables/batch_impact_summary.tex <==
\begin{forest}
for tree={%
    thick,
    drop shadow,
    l sep=0.6cm,
    s sep=0.8cm,
    node options={draw,font=\sffamily},
    edge={semithick,-Latex},
    where level=0{parent}{},
    where level=1{
        minimum height=1cm,
        child,
        parent anchor=south west,
        tier=p,
        l sep=0.25cm,
        for descendants={%
            grandchild,
            minimum height=0.6cm,
            anchor=150,
            edge path={
                \noexpand\path[\forestoption{edge}]
                (!to tier=p.parent anchor) |-(.child anchor)\forestoption{edge label};
            },
        }
    }{},
}
[Batch\\Size
    [High
        [Maximize Throughput
            [Mostly compute-bounded operations
                [Large KV Caches
                    [Latency $\propto$ batch size]
                ]
            ]
        ]
    ]
    [Low
        [Minimize Latency
            [Most operations are memory-bounded
                [Small KV Caches
                    [Latency increases sublinearly.]
                ]
            ]
        ]
    ]
]
\end{forest}

==> Tables/decode_ops.tex <==
\begin{table*}[!t]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Operation   & Input Shapes  & Output Shape & $C_{op}$ & $M_{op}$ \\ \hline
$Q / K / V$ & [B, 1, \underline{$D_{model}$}] $\times$ \textcolor{blue}{[$\underline{D_{model}} , 3D_{model}$]} & B, H, 1, d   & $O(3BD_{model}^2)$ & $O(3D_{model}^2)$\\ \hline
$Q * K^T$  & [B, $1, H, \underline{d}] \times$ \textcolor{red}{$[B, \tau_{cur} + 1, H, \underline{d}]$}  & B, H, 1, $\tau_{cur}+1$   & $O(BH(\tau_{cur}+1)d)$ & $O(B\tau_{cur}D_{model})$ \\ \hline
% $Softmax$                  & B, H, 1, $\tau_{cur}$   & $O(BH\tau_{cur})$  & $O(BH\tau_{cur})$  \\ \hline
$P*V$      & [B, 1, $\underline{\tau_{cur}+1}] \times$ \textcolor{red}{[B, \underline{$\tau_{cur}+1$}, H, d]}  & B, H, 1, d   & $O(BH(\tau_{cur}+1)d)$ & $O(B\tau_{cur} D_{model})$ \\ \hline
$A*W_O$ &  [B, 1, $\underline{D_{model}}] \times $ \textcolor{blue}{[$\underline{D_{model}} , D_{model}$]}  & B, 1,  $D_{model}$      & $O(BD_{model})$  & $O( D_{model}^2)$  \\ \hline
$FF_{up}$ & [B, 1, $\underline{D_{model}}] \times $ \textcolor{blue}{[$\underline{D_{model}} , D_{ff}$]}  & B, 1, $D_{ff}$      & $O(B D_{ff}D_{model})$   & $O( D_{ff}D_{model})$  \\ \hline
$FF_{gate}$ & [B, 1, $\underline{D_{model}}] \times $ \textcolor{blue}{[$\underline{D_{model}} , D_{ff}$]}     & B, 1, $D_{ff}$      & $O(B D_{ff}D_{model})$   & $O( D_{ff}D_{model})$\\ \hline
$FF_{down}$ & [B,1, $\underline{D_{ff}}] \times $ \textcolor{blue}{[$\underline{D_{ff}} , D_{model}$]} & B, 1, $D_{model}$      & $O(B D_{ff}D_{model})$   & $O( D_{ff}D_{model})$\\ \hline
\end{tabular}
\caption{Matrix Multiplication operations during the \textbf{decode} stage. Reduction dimensions are underscored. Blue and red colored operators are model weights and KV caches respectively. $\tau_{cur}$ is sum of prefill tokens($\tau_{p}$) and token generated by LLM before the current token.}
\vspace{-1em}
    \label{tab:decode_ops}
\end{table*}



==> Tables/new_systems_for_various_usecases.tex <==
% Notebook 5. Various model requirement analysis.ipynb


\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Specialized\\  System\end{tabular} & Compute:Mem BW & Compute: Mem Cap & \begin{tabular}[c]{@{}c@{}}Computation\\ (TFLOPs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Memory BW\\ (TB/s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Memory Capacity\\ (GB)\end{tabular} \\ \hline
Sys\_QA & 250 & 20 & 300 & 0.6 & 16 \\ \hline
Sys\_Chat & 500 & 50 & 900 & 3.6 & 16 \\ \hline
Sys\_RAG\_QA & 700 & 70 & 1800 & 2.5 & 24 \\ \hline
Sys\_Summ & 400 & 15 & 750 & 1.875 & 48 \\ \hline
Sys\_Code & 800 & 45 & 1000 & 1.25 & 24 \\ \hline
\end{tabular}
\end{table}

==> Tables/parameter_impact_experiments.tex <==
\begin{table}[h]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\# Batch & \# Beam & \begin{tabular}[c]{@{}c@{}}Input \\ Tokens\end{tabular} & \begin{tabular}[c]{@{}c@{}}Output\\ Tokens\end{tabular} & \begin{tabular}[c]{@{}c@{}}Data\\ Format\end{tabular}  & Experiment \\ \hline
1:32 & * & 2000 & 256 & fp8 & \autoref{fig:beamscaling_trend} \\ \hline
1:32 & 4 & * & 256 & fp8 & \autoref{fig:input_tokens_trend} \\ \hline
1:32 & 4 & 2000 & * & fp8 & \autoref{fig:output_tokens_trend} \\ \hline
1:32 & 4 & 2000 & 256 & * & \autoref{fig:quantization_trend} \\ \hline
\end{tabular}
\label{tab:workload_exp}
\caption{Studies to understand the effect of changing workload parameters.}
\end{table}

==> Tables/prefill_ops.tex <==
% \begin{table*}[!b]
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
% Operation                     & Output Shape & Flops       & Memory Operations    \\ \hline
% $X\_i$ * $\{W\_Q, W\_k, W\_v\}$ & B, h, $\tau_{p}$, d   & $O(3B\tau_{p}D^2)$ & $O(4B\tau_{p}D + 3D^2)$   \\ \hline
% $Q * K^T$                     & B, h, $\tau_{p}$, $\tau_{p}$   & $O(BhL^2d)$ & $O(2B\tau_{p}D + BhL^2)$  \\ \hline
% $Softmax(V)$                  & B, h, $\tau_{p}$, $\tau_{p}$   & $O(BhL^2)$  & $O(2BhL^2)$            \\ \hline
% $P*V$                         & B, h, $\tau_{p}$, d   & $O(BhL^2d)$ & $O(2B\tau_{p}D + BhL^2)$    \\ \hline
% $A*W_O$                       & B, $\tau_{p}$, D      & $O(B\tau_{p}D^2)$  & $O(B\tau_{p}D + D^2)$      \\ \hline
% $FF_{up}  : X_{ff} * W_{up}$     & B, $\tau_{p}$, F      & $O(B\tau_{p}DF)$   & $O(B\tau_{p}D + DF + B\tau_{p}F)$  \\ \hline
% $FF_{gate}\footnote{Not present in GPT3-175B}  : X_{ff} * W_{gate}$     & B, $\tau_{p}$, F      & $O(B\tau_{p}DF)$   & $O(B\tau_{p}D + DF + B\tau_{p}F)$ \\ \hline
% $FF_{down}  : X_{hidden} * W_{down}$ & B, $\tau_{p}$, D      & $O(B\tau_{p}DF)$   & $O(B\tau_{p}F + FD + B\tau_{p}D)$  \\ \hline
% \end{tabular}
% \caption{Various operations, their FLOPs calculations, and Memory Operations during the prefill phase.}
%     \label{tab:prefill_ops}
% \end{table*}

\begin{table*}[!t]
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|c|}
\hline
Operation      & Input Shapes               & Output Shape & $C_{op}$       & $M_{op}$    \\ \hline
$Q/K/V$ & [B, $\tau_{p}$, $\underline{D_{model}}] \times $ \textcolor{blue}{[$\underline{D_{model}} , 3D_{model}$]}  & 3B, $\tau_{p}, H, d$   & $O(3B\tau_{p}D_{model}^2)$ & $O(4B\tau_{p}D_{model} + 3D_{model}^2)$   \\ \hline
$Q * K^T$  & [B, $\tau_{p}, H, \underline{d}] \times [B, \tau_{p}, H, \underline{d}]$  & B, H, $\tau_{p}$, $\tau_{p}$   & $O(BH\tau_{p}^2d)$ & $O(2B\tau_{p}D_{model} + BH\tau_{p}^2)$  \\ \hline
% $Softmax$              &    & B, H, $\tau_{p}$, $\tau_{p}$   & $O(BH\tau_{p}^2)$  & $O(2BH\tau_{p}\tau_{p}^2)$            \\ \hline
$P*V$      & [B, $\tau_{p}$, $\underline{\tau_{p}}] \times [B, \underline{\tau_{p}}$, H, d]      & B, H, $\tau_{p}$, d   & $O(BH\tau_{p}^2d)$ & $O(2B\tau_{p}D_{model} + BH\tau_{p}^2)$    \\ \hline
$A*W_O$                &  [B, $\tau_{p}$, $\underline{D_{model}}] \times $ \textcolor{blue}{[$\underline{D_{model}} , D_{model}$]}      & B, $\tau_{p}$, $D_{model}$      & $O(B\tau_{p}D_{model}^2)$  & $O(B\tau_{p}D_{model} + D_{model}^2)$      \\ \hline
$FF_{up}$ & [B, $\tau_{p}$, $\underline{D_{model}}] \times $ \textcolor{blue}{[$\underline{D_{model}} , D_{ff}$]}    & B, $\tau_{p}$, $D_{ff}$      & $O(B\tau_{p}D_{model}D_{ff})$   & $O(B\tau_{p}D_{model} + D_{model}D_{ff} + B\tau_{p}D_{ff})$  \\ \hline
$FF_{gate}$ & [B, $\tau_{p}$, $\underline{D_{model}}] \times $ \textcolor{blue}{[$\underline{D_{model}} , D_{ff}$]}  &B, $\tau_{p}$, $D_{ff}$      & $O(B\tau_{p}D_{model}D_{ff})$   & $O(B\tau_{p}D_{model} + D_{model}D_{ff} + B\tau_{p}D_{ff})$ \\ \hline
$FF_{down}$ & [B, $\tau_{p}$, $\underline{D_{ff}}] \times $ \textcolor{blue}{[$\underline{D_{ff}} , D_{model}$]}  &B, $\tau_{p}$, $D_{model}$     & $O(B\tau_{p}D_{model}D_{ff})$   & $O(B\tau_{p}D_{ff} + D_{ff}D_{model} + B\tau_{p}D_{model})$  \\ \hline
\end{tabular}
\caption{Matrix Multiplication operations during the \textbf{prefill} stage. Reduction dimensions are underscored. Blue colored operators are model weights.
}
\vspace{-1em}
    \label{tab:prefill_ops}
\end{table*}



==> _MICRO_25__GenZ/micro58/shorthands.tex <==

\usetikzlibrary{shadows, arrows.meta}

% \usepackage[table,xcdraw]{xcolor}

\tikzset{parent/.style={align=center,text width=2cm,fill=green!20,rounded corners=2pt},
    child/.style={align=center,text width=2.8cm,fill=green!50,rounded corners=6pt},
    grandchild/.style={fill=pink!50,text width=2.3cm}
}


\newcommand{\SubItem}[1]{
    {\setlength\itemindent{15pt} \item[-] #1}
}
\newcommand{\abc}{{\sf abc}\xspace}
\newcommand{\dse}{{\sf dse}\xspace}
\newcommand{\defns}{{\sf def}}
\newcommand{\tool}{{GenZ }}
\newcommand{\toolns}{{GenZ}}

\newcommand{\AB}[1]{{\color{magenta}\bfseries [Abhi:: #1]}}
\newcommand{\RR}[1]{{\color{purple}\bfseries [Ritik:: #1]}} 
\newcommand{\GJ}[1]{{\color{blue}\bfseries [Geonhwa:: #1]}} 
\newcommand{\SudS}[1]{{\color{orange}\bfseries [Sudarshan:: #1]}}
\newcommand{\SK}[1]{{\color{purple}\bfseries [Souvik:: #1]}} 
\newcommand{\TK}[1]{{\color{red}\bfseries [Tushar:: #1]}}
\newcommand{\TODO}[1]{\textcolor{red}{TODO:: #1}}
\newcommand{\rev}[1]{\textcolor{blue}{#1}}
\newcommand{\fixme}[1]{\textcolor{red}{#1 \textit{- FIXME}}}

% If you want to remove all comments remove #1.
% \newcommand{\com}[1]{\textbf{\textcolor{orange}{#1}}}
\newcommand{\niparagraph}[1]{\vspace{1pt}\noindent\textbf{#1}}
\newcommand{\checkbox}{\textbf{\textcolor{green}{\ding{51}}}}
\newcommand{\xbox}{\textbf{\textcolor{red}{\ding{55}}}}



\newcommand*\hcircled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=2pt] (char) {#1};}}


% \newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,fill=black,text=white,font=\sffamily\bfseries\small, inner sep=1.2pt] (char) {#1};}}

            
% Sections
% \def\Snospace~{\S{}}
% \renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section} \def\subsubsectionautorefname{Section }

\def\figureautorefname{Fig.}

\definecolor{turqoise}{HTML}{4BCAD2}
\definecolor{orangered}{HTML}{CF1040}
\definecolor{redgreen}{HTML}{66AA00}
% Define the five rev colors
\definecolor{lightgray}{gray}{0.9}

==> includes/cmds.tex <==
\newcommand{\circleNumber}[1]{
{\large \textcircled{\small #1}} }

%%%%%%%%%%%%%%%%%%%% Figure commands %%%%%%%%%%%%%%%%%%%% 
% \newcommand{\insertFigure}[2]{
%     \begin{figure}[t]
% \setlength{\abovecaptionskip}{-3pt}
% \setlength{\belowcaptionskip}{-1pt}
%         \centering
%         \includegraphics[width=\linewidth]{\FIGDIR/#1}
% 	\vspace{-2mm}
%         \caption{#2}
% 	\vspace{-2mm}
%         \label{fig:#1}
%     \end{figure}
% }

% \newcommand{\insertWideFigure}[2]{
%     \begin{figure*}
% \setlength{\abovecaptionskip}{-3pt}
% \setlength{\belowcaptionskip}{-1pt}
%         \centering
%         \includegraphics[width=\textwidth]{\FIGDIR/#1}
% 	\vspace{-2mm}
%         \caption{#2}
% 	\vspace{-2mm}
%         \label{fig:#1}
%     \end{figure*}
% }
%\newcommand{\insertWideFigure}[2]{
%    \begin{figure*}[h]
%    \setlength{\abovecaptionskip}{-2pt}
%    \setlength{\belowcaptionskip}{-4pt}
%        \centering
%        \includegraphics[width=\textwidth]{\FIGDIR/#1.pdf}
%	    \vspace{-3mm}
%        \caption{\small #2}
%    	\vspace{-2mm}
%        \label{fig:#1}
%    \end{figure*}
%}

%\newcommand{\matmul}{\textsc{tdpbf16ps}\xspace}
\newcommand{\tileload}{\textit{tileload}\xspace}
\newcommand{\tilestore}{\textit{tilestore}\xspace}
\newcommand{\matmul}{\textit{tdpbf16ps}\xspace}

\newcommand{\rasatl}{\textit{rasa\_tl}\xspace}
\newcommand{\rasats}{\textit{rasa\_ts}\xspace}
\newcommand{\rasamm}{\textit{rasa\_mm}\xspace}

%\newcommnad{\matmul}{\textit{tdpbf16ps}}

%%%%%%%%%%%%%%%%%%%%  TODO commands %%%%%%%%%%%%%%%%%%%% 




==> includes/packages.tex <==
\input{includes/cmds}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{amssymb}
\usepackage{algorithmic}
\usepackage{textcomp}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{textcomp}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{tabularray}
\usepackage{array, makecell}

\usepackage{float}
% \usepackage[hyphens]{url}
\usepackage{fancyhdr}
\usepackage{colortbl}
\usepackage{arydshln}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{soul}
\usepackage{hyperref}
\usepackage{tcolorbox}
\usepackage{wrapfig}
\usepackage{algorithm2e}
\RestyleAlgo{ruled} 
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{tikz}
\usepackage{float}
% Include other packages here, before hyperref.
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{cleveref}
\crefformat{section}{\S#2#1#3} % see manual of cleveref, section 8.2.1
\crefformat{subsection}{\S#2#1#3}
\crefformat{subsubsection}{\S#2#1#3}

\usepackage{hyperref}
\usepackage{microtype}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables

% Added by abhi


\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{cite}
% \usepackage{amssymb}
\usepackage{amsmath,amsfonts}
\usepackage{newtxtext,newtxmath}
\usepackage{algorithmic}
\usepackage{textcomp}
\usepackage{comment}
\usepackage{algorithm2e}
\usepackage{fancyhdr}
\usepackage{lipsum}
\usepackage{comment}
\usepackage{outlines}
\usepackage{graphicx}
\usepackage{float}
% \usepackage[most]{tcolorbox}
% \usepackage{tabularx}
\usepackage{tablefootnote}
\usepackage[export]{adjustbox}

\usepackage{multirow}
\usepackage{pifont}% http://ctan.org/pkg/pifont


\usepackage{subcaption}
% \expandafter\def\csname ver@subfig.sty\endcsname{}


\usepackage{svg}
\usepackage{hyperref}

% \usepackage{subfig}
\usepackage{forest}

\newcommand{\tick}{\includegraphics[height=1.5ex]{figures/checked.png}}
\newcommand{\cross}{\includegraphics[height=1.5ex]{figures/delete.png}}
\newcommand{\exclamation}{\includegraphics[height=1.5ex]{figures/exclamation-2.png}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,fill,inner sep=0pt] (char) {\textcolor{white}{#1}};}}

\definecolor{revA}{HTML}{000000}%{FF5733} % A reddish-orange
\definecolor{revB}{HTML}{000000}%{33CC57} % A green shade
\definecolor{revC}{HTML}{000000}%{3357FF} % A blue shade
\definecolor{revD}{HTML}{000000}%{FF33A1} % A pinkish shade
\definecolor{revE}{HTML}{000000}%{A133FF} % A purple shade

\definecolor{colorRevA}{rgb}{0.85, 0.90, 0.98}
\definecolor{colorRevB}{rgb}{0.97, 0.80, 0.796}
\definecolor{colorRevC}{rgb}{0.87, 0.83, 0.90}
\definecolor{colorRevD}{rgb}{0.83, 0.91, 0.83}
\definecolor{colorRevE}{rgb}{1, 0.90, 0.80}
\definecolor{blond}{rgb}{0.98, 0.94, 0.75}

\newcommand{\colorciteB}[1]{\tcbox[colframe=colorRevB, colback=colorRevB, boxrule=0mm, arc=0mm, left=0mm, right=0mm, top=0mm, bottom=0mm, boxsep=0pt, on line]{\cite{#1}}}

\newcommand{\colorrefA}[1]{\tcbox[colframe=colorRevA, colback=colorRevA, boxrule=0mm, arc=0mm, left=0mm, right=0mm, top=0mm, bottom=0mm, boxsep=0pt, on line]{\cref{#1}}}

\newcommand{\colorciteA}[1]{\tcbox[colframe=colorRevA, colback=colorRevA, boxrule=0mm, arc=0mm, left=0mm, right=0mm, top=0mm, bottom=0mm, boxsep=0pt, on line]{\cite{#1}}}

\DeclareRobustCommand{\RevA}[1]{{\sethlcolor{colorRevA}\hl{#1}}}
\DeclareRobustCommand{\RevB}[1]{{\sethlcolor{colorRevB}\hl{#1}}}
\DeclareRobustCommand{\RevC}[1]{{\sethlcolor{colorRevC}\hl{#1}}}
\DeclareRobustCommand{\RevD}[1]{{\sethlcolor{colorRevD}\hl{#1}}}
\DeclareRobustCommand{\RevE}[1]{{\sethlcolor{colorRevE}\hl{#1}}}
\DeclareRobustCommand{\RevCom}[1]{{\sethlcolor{blond}\hl{#1}}}

\newcommand{\titleRev}[2]{
    \texorpdfstring{{\sethlcolor{#2}\hl{#1}}}{#1}
}
